Stochastic Scene-Aware Motion Prediction

A long-standing goal in computer vision is to capture, model, and realistically synthesize human behavior. Specifically, by learning from data, our goal is to enable virtual humans to navigate within cluttered indoor scenes and naturally interact with objects. Such embodied behavior has applications in virtual reality, computer games, and robotics, while synthesized behavior can be used as a source of training data. This is challenging because real human motion is diverse and adapts to the scene. For example, a person can sit or lie on a sofa in many places and with varying styles. It is necessary to model this diversity when synthesizing virtual humans that realistically perform human-scene interactions. We present a novel data-driven, stochastic motion synthesis method that models different styles of performing a given action with a target object. Our method, called SAMP, for Scene-Aware Motion Prediction, generalizes to target objects of various geometries while enabling the character to navigate in cluttered scenes. To train our method, we collected MoCap data covering various sitting, lying down, walking, and running styles. We demonstrate our method on complex indoor scenes and achieve superior performance compared to existing solutions. Our code and data are available for research at https://samp.is.tue.mpg.de.

==> FIG_foot_sliding.tex <==
\begin{figure}
	\centering	
	\includegraphics[width=\linewidth]{example-image-a}	
	\caption{
	Foot sliding.
	}
	\label{fig:foot_sliding}
\end{figure}

==> FIG_gen_locomotion.tex <==
\begin{figure}
	\centering	
	\includegraphics[width=\linewidth]{figures/gen_locomotion.png}	
	\caption{
	Generated running and walking motion. The user controls the motion by providing start/stop signal and the motion direction using the keyboard.
	}
	\label{fig:gen_locomotion}
\end{figure}

==> FIG_gen_lying_down.tex <==
\begin{figure}
	\centering	
	\includegraphics[width=\linewidth]{figures/gen_lyingdown.png}
	\vspace{-0.25in}
	\caption{Different lying Down examples generated by \modelname.}
	\label{fig:gen_lyingdown}
\end{figure}

==> FIG_ours_vs_nsm_1.tex <==
\begin{figure}
	\centering	
	\includegraphics[width=\linewidth]{example-image-a}	
	\caption{
	Ours vs \nsm. Our method is capable of generating diverse results while \nsm is a deterministic model generating the same result every time.
	}
	\label{fig:ours_vs_nsm_1}
\end{figure}

==> FIG_path_planning.tex <==
\begin{figure}
	\centering	
	\includegraphics[width=\linewidth]{figures/path_planning.png}	
	\vspace{-0.1in}
	\caption{
	A* is used to compute an obstacle free path between the character starting position and the goal. The walk-able areas are shown in blue.
	}
	\label{fig:path_planning}
\end{figure}

==> TAB_penetration.tex <==
\begin{table}[]
\centering
\begin{tabular}{c|c}
\hline
Model                  & Penetrating Frames  \\ \hline
\nsm                    &             \\
\modelname w/o path planning &      18       \\
\modelname with path planning &      2      
\end{tabular}
\caption{Average number of penetrating frames.}
\label{tab:penetration}
\end{table}
